Bug Analysis Towards Bug Resolution Time Prediction

Bugs are inevitable in software development, and their reporting in open repositories can enhance software transparency and reliability assessment. This study aims to extract information from the issue tracking system Jira and proposes a methodology to estimate resolution time for new bugs. The methodology is applied to network project ONAP, addressing concerns of network operators and manufacturers. This research provides insights into bug resolution times and related aspects in network softwarization projects.

==> 03_background.tex <==
\section{Related Work Yagiz and Poul?}
\label{sec:background}

\yagiz{rewrite from scratch for the same papers and add if can find time}

This section will discuss previous works on bug data analysis and bug resolution processes. %Also, the methodology used in this work will be explained. 

Issue tracking systems are mined, and researchers of \cite{ortu2015jira} use this process to offer the dataset of all the issues from different projects. Additionally, the authors of \cite{vieira2019reports} conduct various analyses of the collected data, which comes from 55 different Apache projects. These 55 projects are classified into 9 categories, such as big data, security, and libraries. The authors examine the percentage of fields that change the reporting of the bugs. They define bug resolution duration time from the creation and closure of a bug as a bug-fix effort and compare the bug resolution times across different project categories. Additionally, they investigate when the priority and assignee are defined and analyze the number of bugs in which these values change after the initial bug report. Furthermore, the study delves into the changes in bug status, analyzing the percentage of bugs transitioning between states. This dataset is used in this work. As the primary contribution of this work is the provided dataset, it does not delve into a comprehensive analysis or propose a methodology to estimate bug resolution duration. In addition to the self-collected data, the bug reports from \cite{vieira2019reports} are also examined in this study.

The authors investigate the impact of bug attributes such as reporter and priority on the time it takes to resolve them in the study \cite{zhang2013predicting}. The used data in this work is not publicly accessible. They employed the K-nearest neighbour algorithm to predict the resolution time of bugs. Based on these attributes from the issue-tracking system, they predicted whether a bug would be resolved quickly or slowly. The authors of \cite{akbarinasaji2018predicting} replicated the study presented in \cite{zhang2013predicting}, but they utilized open-source data sourced from Bugzilla Firefox. Both studies concluded that the identity of the reporter or assignee is more crucial than the bug's priority. However, a weakness of these predictions is that they are binary (quick or slow) rather than numerical. 

Furthermore, their proposal incorporates a Markov-based approach to estimate the number of bugs that can be resolved within a specific timeframe. They also employ a Monte Carlo-based method to predict the overall time required to fix a given quantity of bugs. The time is divided into months, and they estimate the percentage of bugs that will be resolved within a particular time period. It is important to note that the Markov-based model they used does not focus on examining the solution process of individual bugs as separate entities but rather on determining the percentage of bugs in different states after a certain period of time, measured in months.



% The bug reports from three projects of CA Technologies were analyzed by \cite{zhang2013predicting}, encompassing reports submitted by both CA Technologies' engineers and their customers. Their proposal involves a Markov-based approach to estimate the number of bugs that can be resolved within a specific timeframe and a Monte Carlo-based method for predicting the overall time needed to fix a given number of bugs. Furthermore, they provide predictions regarding whether a bug will be resolved quickly or slowly depending on bug information from the issue-tracking system. The data utilized in this study is not publicly available, and the prediction of resolution time is binary rather than a numerical value, classified as either quick or slow.

%Authors of \cite{akbarinasaji2018predicting} conducted a replication study of \cite{zhang2013predicting} using open-source data from Bugzilla Firefox. The authors employed the same models and similarly predicted the resolution time as either quick or slow. Both of these studies reach the conclusion that the priority of a bug is not as crucial as the identity of the reporter or assignee. While their dataset is publicly available, they also arrived at a binary conclusion regarding bug resolution time instead of providing a numerical value.


%Issue tracking systems are mined and the dataset as a result of this process is offered by different researchers \cite{ortu2015jira, vieira2019reports}. The dataset from \cite{ortu2015jira} encompasses all issues derived from four open-source ecosystems. This dataset comprises 700,000 issues and 2 million comments. The main contribution of the paper lies in providing the dataset itself, without presenting any specific results. They also investigate the comments that contain emotions and the impact of these emotions on issue-fixing time. It is worth noting that the data was collected prior to 2015, implying that the bug resolution process at that time may differ from the present.


%The dataset presented in \cite{vieira2019reports} pertains to the year 2019 and encompasses 10 years of bug reports from 55 Apache projects. Along with providing the dataset, the authors conduct various analyses of the collected data. These 55 projects are classified into 9 distinct categories, such as big data, security, and libraries. The authors examine the percentage of fields that undergo changes after the reporting of the bugs.  They define bug resolution duration time from the creation and closure of a bug as bug-fix effort and compare the bug resolution times across different project categories. Additionally, they investigate when the priority and assignee are defined, and also analyze the number of bugs in which these values change after the initial bug report. Furthermore, the study delves into the changes in bug status, analyzing the percentage of bugs transitioning between states. This dataset is used in this work. As the primary contribution of this work is the provided dataset, it does not delve into a comprehensive analysis and does not propose a methodology to estimate bug resolution duration. In addition to the self-collected data, the bug reports from this dataset are also examined in this study.

%A bug is an error in the normal work of software and causes the software to operate in an unexpected way. Bugs can cause minor errors like typos or major errors like a total system crash \cite{khleel2021comprehensive}. Bugs can appear because of many different reasons like coding errors and wrong logic. Dealing with appearing bugs is an important part of the software development process \cite{vieira2019reports}. Different techniques like testing or code review. Nowadays issue tracking systems like Jira and Bugzilla are used to organize software development and organize the bug-solving process. With time these issue tracking systems become a very handful tool to understand the handling process of appearing bugs.

%Issue tracking systems are mined and the dataset as a result of this process is offered by different researchers \cite{vieira2019reports, ortu2015jira}. These datasets are used to investigate different aspects of bugs solving process. As an example the impact of continuous delivery adaption on bug solving duration is studied in \cite{de2022studying}. 

%Yagiz on data repositories, data analysis.\\

%Poul on models.

==> 04_predictionmodel.old.tex <==
\section{State model of Software Bug Recovery Poul?}
\label{sec:model}

The model is inspired by \textit{Escalating recovery}~\cite{Heegaard:2015} and using \textit{response time blocks}~\cite{Grottke:2008}. Since our data contains (i) $t_{\tt ij}$, time for transition from state $i$ to $j$, and (ii) $n_{\tt ij}$, number of transitions from state $i$ to $j$, we use a \textit{dual state model}, where transitions are vertices and states are arcs.
\subsection{Software bug recovery stages/annotations}
Description of possible stages identified in ONAP bug reports. All start with \textit{Open}, but the remaining sequence varies, and not all stages are in all reports. We have defined \textit{Closed} as the final (absorbing) stage, i.e., no actions are take after that.
\begin{enumerate}
    \item \textit{Open} - all tickets start here
    \item \textit{InProgress} - 
    \item \textit{Submitted} - 
    \item \textit{Delivered} - 
    \item \textit{Closed} - all tickets ends here (the data set is modified)
    \item \textit{Reopened} -
    \item \textit{Implemented} - 
    \item \textit{Done} -
    \item \textit{ToDo} - this stage is removed from the data set due to too few observations.
\end{enumerate}
Classification of severeness...
\begin{itemize}
    \item Serious ++
\end{itemize}
Data extracted
\begin{itemize}
    \item $t_{ij}$ - average transition time from state/stage $i$ to $j$.
    \item $n_{ij}$ - number of transitions from state/stage $i$ to $j$.
\end{itemize}

\subsection{Software bug recovery models}
A state model of the bug recovery stages by defining either the stages or the transitions between stages as \textit{states}.  In this section we do both, starting with defining $\Omega = \{ \omega_{i} \}$ as the set of states, where $\omega_{i}$ is either stage $i$ in the bug report, or  $\omega_{i} = \tau_{kl}$ is the transition from stage $k$ to $l$ in the \textit{dual model}. The nodes in the state model is described by $\omega_{i}$, while the edges are either the stage transitions ($\tau_{ij}$), or in the dual model, connecting a stage transitions ($\tau_{ij} \rightarrow \tau_{jx};\; \forall x$).

As a simple example, consider a software recovery process with four bug stages \textit{Open}~(O), \textit{InProgress}~(I), `\textit{On Hold}~(H), and \textit{Close}~(C).  In Fig.~\ref{fig:state-model}, The state model has four states, $\Omega =\{O,I,H,C\}$, and six transitions, 
$T = \{ \tau_{\tt OI}, \tau_{\tt OH}, \tau_{\tt HO},\tau_{\tt IH},\tau_{\tt HC},\tau_{\tt IC}\}$.
% as illustrated in Fig.~\ref{fig:dual-del}. 
%
\begin{figure}
     \centering
     \includegraphics[width=\columnwidth]{figs/state-model.pdf}
     \caption{Software Bug Recovery State Model Example}\label{fig:state-model}
\end{figure}
%
The dual model in Fig.~\ref{fig:dual-del} is established by first defining the transitions in the state model as nodes, %see Fig.~\ref{fig:dual-del}. 
where the states are ``collapsed'', and the transitions between the nodes are replaced. The final model is shown in Fig.\ref{fig:dual-final}. This is the Continuous Time Markov Chain (CTMC) model that will be applied in the following section.  The assigned rates in Fig.\ref{fig:dual-final} are explained in the \textit{response block approach} in the following subsection~\ref{sec:resp-block}.
%
\begin{figure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/dual-model-delstate.pdf}
         \caption{Dual model: vertices added and states are collapsed into arcs}
         \label{fig:dual-del}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/dual-model-final.pdf}
         \caption{Dual model: final model with parameters}
         \label{fig:dual-final}
     \end{subfigure}
     \caption{Dual model of software bug resolve}
     \label{fig:bug-resolve}
\end{figure}

% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/state-model.pdf}
%           \caption{State model}
%           \label{fig:state-model}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/dual-model-addtrans.pdf}
%          \caption{Dual model: vertices added on transition}
%          \label{fig:dual-add}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/dual-model-delstate.pdf}
%          \caption{Dual model: states are collapsed into arcs}
%          \label{fig:dual-del}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/dual-model-final.pdf}
%          \caption{Dual model: final model with parameters}
%          \label{fig:dual-final}
%      \end{subfigure}
%      \caption{Dual model of software bug resolve}
%      \label{fig:bug-resolve}
% \end{figure*}

\subsection{Software bug resolve time distribution}\label{sec:resp-block}
To evaluate the bug resolve time distribution, we apply the \textit{response time block approach} described in~\cite{Trivedi:2001,Grottke:2008}. 
The basic idea is to construct a CTMC, connecting the source (src - opening of a bug report) to the destination (dst - closing of a bug report). The states in this CTMC is the time from one annotation to the next in resolving the bug, as illustrated in the ``dual model'' in Fig.~\ref{fig:dual-final}.  The transient probability of the absorbing state in CTMC (dst) is then the CDF of the time from ${\tt src}\rightarrow{\tt dst}$, i.e. the resolve time.
In this paper, we assume that the service of a bug in each of the states are not constrained, such that each state is an M/M/$\infty$-queue, and hence the bug arrival intensity is not relevant.  Approximations for other Markovian, and non-Markovian networks also exist, see~\cite{Grottke:2008} for details. 

In this section we apply the block method to bug resolve time. 
The ``stochastic routing'' in our model is the probability $r_{ij}$ that a bug fix phase $i$ is followed by $j$, given in a routing matrix, $\mathcal{R}=\{r_{ij}\}$.
The method is presented in four steps.
\begin{enumerate}
\item Create a CTMC, $\Omega=\{\omega_{\tt 0},\omega_{1}, \cdots, \omega_{m}, \omega_{\tt m+1}\}$, with nodes (states) where $\omega_{\tt 0} = \omega_{S1}$ is the initialisation of the bug report, and $\omega_{\tt m+1} = \omega_{5D}$ is the absorbing node where the bug has been resolved (see description of the data set in the following section). $\omega_{i}$ is node $i$ in the dual model in Fig.~\ref{fig:dual-final}. The CTMC has $m+2$ nodes where $m$ is the number of possible transitions in the original ONAP state model in Fig.~\ref{fig:ONAP}.  The node in the dual model is the transition between two states in the ONAP state model.
\item The ``response'' time distribution in node $i$ is represented
by an exponential distribution with service rate $\mu_{i}$ of node $i$, since we have assumed an M/M/$\infty$-queue in each node). The generator matrix $\mathcal{Q}$ of the CTMC is then constructed by:
\begin{enumerate}
    \item The ``routing'' from node $i$ to $j$ is $Q_{\omega_{i}\omega_{j}} = \mu_{i} r_{ij}$. The probabilities is estimated by $r_{ij} = n_{ij}/\sum_{j=1}^m n_{ij}$
    \item The exit is at the dst $i=d$, with $Q_{\omega_{i}\omega_{d}}=\mu_{i}r_{id}$.
    \item All other entries are $0$ except the diagonals,\\ $Q_{\omega_{i}\omega_{i}}=-\sum_{\omega_{j}\in \Omega, \omega_{j}\ne \omega_{i}}Q_{\omega_{i}\omega_{j}}$.
\end{enumerate}
\item The cumulative resolve time distribution function is equal to the probability $P_{\mathcal{Q}}(\omega_{d};t)$ of being in the absorbing state $\omega_{5d}$ at time $t$ under the generator matrix~$\mathcal{Q}$. The probabilities $P_{\mathcal{Q}}(\omega;t)$,
$\omega \in \Omega$ are found by solving $\mathbf{P}_{\mathcal{Q}}(t)=\{P_{\mathcal{Q}}(\omega;t)\}$,
\[
    \frac{d}{du}\mathbf{P}_{\mathbf{Q}}(t)=\mathbf{P}_{\mathbf{Q}}(t)\cdot\mathbf{Q}
\]
The initial conditions are $P_{\mathbf{Q}}(\omega;0)=1$ with $\omega={\tt S1}$, and $P_{\mathbf{Q}}(\omega;0)=0$ for all other nodes.
\end{enumerate}

With non-Exponential service time assumptions (in $M/M/\infty$) the approach is approximate. The non-Exponential service times can be approximated by \textit{phase-type} distribution. 
More details on this method and generalization to $M/M/c/b$-queues and non-Markovian networks are found in~\cite{Grottke:2008}.

==> 05_case-study.tex <==
\section{Discussion}
\label{sec:cases}


\subsection{Factors influencing bug resolving time}

\subsubsection{Bug Priority Level}

Bug priority is a way to categorize bugs based on their severity and impact on the system .It helps the development team prioritize which bugs to fix first and which can be addressed later. Projects have different naming for priorities and we distribute priority levels from 1 to 5, with 1 being the highest priority and 5 being the lowest. A bug with a high priority level (e.g., priority 1) is considered more critical and needs to be fixed as soon as possible, while bugs with lower priority levels may be addressed later. The priority level is usually set by the reporter of the bug or the project manager, and it can be updated as the bug progresses through the workflow.

\subsubsection{Assignee and Creator}

The "assignee" is the person who is responsible for working on a particular issue or task. They are the person who is expected to take action on the issue, such as fixing a bug or implementing a new feature. The "creator" is the person who created the issue in Jira. They are the person who reported the bug or requested the new feature.

\subsection{Deviation of real workflow from specified workflow}

RQ2

%\subsection{Modeling the bug resolving process with a Markov Model}

RQ3

\subsection{Importance of workflow stages for bug resolving time}

RQ4

Describe the data we can extract from the tickets/bug reports.

Map the recovery stage annotations in the bug reports to the notation from the previous section, $t_{ij}$, $n_{ij}$, and $p_{ij}$.  Assign numbers to the 8 states.
$\Omega =\{ 1 ({\tt Open}), \cdots\}$.

\poul{Need to include a discussion about the reliability of the data, the uncertainties in how the software engineers - bug fixers - are using the annotations.  We need to describe how we select data (ongoing vs completed tickets/bug reports), explain the approach outlined in the supervision meeting 2022-11-09.}

\begin{itemize}
    \item pie diagram on the percentage of bugs which end in Done state
    \item developers demographic distribution as extra info: graph of bugs and developers according to the criticality of the bug
    \item information on how the debuggers follow the proposed states shown in Section 3
    \item time distribution at the different states
\end{itemize}

\subsection{ONAP recovery statistics}

Data from severe bugs (from period ??) 
\begin{table}[htb]
    \small
    \centering
    \caption{ONAP: data from bug reports}
    \label{tab:data}

    \begin{tabular}[width=\columnwidth]{llll}
    \toprule
         From & To & Time & Number \\
         \midrule
         Open & InProgress & 113.85 & 727\\
         Open & Closed & 231.06  & 161\\
         Open & Delivered & 280.72 & 111\\
         Open & Done & 676.35 & 38\\
         InProgress & Submitted & 57.13 & 623\\
         InProgress & Closed & 351.54 & 114\\
         InProgress & Open & 209.39 & 38\\
         InProgress & Done & 126.98 & 54\\
         InProgress & Implemented & 23.12 & 51\\
         Submitted & Delivered & 43.98 & 578\\
         Submitted & InProgress & 116.03 & 43\\
         Delivered & Closed & 75.69 & 631\\
         Delivered & Reopened & 49.1  & 82\\
         \color{gray}{Closed} & \color{gray}{Reopened} & \color{gray}{427.91} & \color{gray}{73}\\
         Reopened & InProgress & 37.72 & 99\\
         Reopened & Closed & 117.43 & 29\\
         \color{gray}{Reopened} & \color{gray}{Delivered} & \color{gray}{60.25} & \color{gray}{26}\\
         Implemented & Done & 31.41 & 50\\
         Done & Closed & 4190.62 & 131\\
         \bottomrule
    \end{tabular}
\end{table}


% \subsection{ONAP simulation model}
% Should we also include simulation? Or is the 

\subsection{ONAP analytic model}
% In Fig.~\ref{fig:ONAP}, the state models describing the 8 possible annotations found in the bug reports in ONAP is shown (the {\em todo} state is removed due to a very low number observations). 
% %
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.85\columnwidth]{figs/ONAP-model.pdf}
%     \caption{ONAP resolve model (remove red transitions)}\label{fig:ONAP}
% \end{figure}

% The model is transformed to the dual model as described in the previous section, seer Fig.~\ref{fig:ONAP-dual}. %(not presented here to save space and for readability?).  
% Note that state 5 (Closed) is made absorbing by removing the transition $5\rightarrow 6$, a small number of transitions. The transition $6\rightarrow 4$ is removed too for the same reason, with no visible consequences for the transient state probabilities, $p_{\omega_{i}}(t)$. 
% %
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/ONAP-dual-model.pdf}
%     \caption{ONAP resolve dual model. 5D is the absorbing node, and the red lines are the transitions to this absorbing node.}\label{fig:ONAP-dual}
% \end{figure}

\subsection{Numerical results}
Results comparing the emiprical data with the analytic model are shown in Fig.~\ref{fig:closed-dist}.  
%The plotted transient probability of node/state $\tt 5D$, $P_{5D}(t)$ is the cumulative distribution function (CDF), $F(t)$ of the software bug resolve time. 
%
% \begin{figure}[htb]
%     \centering
%     \includegraphics[angle=-90,width=\columnwidth]{figs/response-time.pdf}
%     %\caption{Transient probabilities for three of the states in the ONAP case, $p_{10}(t)$ is the cumulative resolve time distribution (CDF)}\label{fig:resp-time}
%     \caption{Cumulative resolve time distribution (CDF)}\label{fig:resp-time}
% \end{figure}

% \begin{figure*}[tb]%
% \centering
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-ONOS, pri=1.pdf}
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-ONAP, pri=1.pdf}
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-Apache,pri=1.pdf}\\
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-ONOS, pri=2.pdf}
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-ONAP, pri=2.pdf}
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-Apache,pri=2.pdf}
% \caption{Comparison of the empirical cumulative resolve time distribution (CDF) the analytic model model for three projects and two priority levels. \poul{Too many, they all show the same, we need to select two (or four?)}}%
% \label{fig:closed-dist}%
% \end{figure*}




==> 06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}


\subsection{Factors influencing bug resolving time}

\subsubsection{Bug Priority Level}

Bug priority is a way to categorize bugs based on their severity and impact on the system. The priority level is usually set by the reporter of the bug or the project manager, and it can be updated as the bug progresses through the workflow.

\subsubsection{Assignee and Reporter}

%In Subsectio~\ref{\label{sec:data}}, we showed that the assignee and reporter have an impact on bug resolution duration. In addition, we also showed that assigning the reporter of the bug reduced the bug-solving duration drastically.  

\subsection{Deviation of real workflow from specified workflow}

RQ2

%\subsection{Modeling the bug resolving process with a Markov Model}

RQ3

\subsection{Importance of workflow stages for bug resolving time}

RQ4

Describe the data we can extract from the tickets/bug reports.

Map the recovery stage annotations in the bug reports to the notation from the previous section, $t_{ij}$, $n_{ij}$, and $p_{ij}$.  Assign numbers to the 8 states.
$\Omega =\{ 1 ({\tt Open}), \cdots\}$.

\poul{Need to include a discussion about the reliability of the data, the uncertainties in how the software engineers - bug fixers - are using the annotations.  We need to describe how we select data (ongoing vs completed tickets/bug reports), explain the approach outlined in the supervision meeting 2022-11-09.}

\begin{itemize}
    \item pie diagram on the percentage of bugs which end in Done state
    \item developers demographic distribution as extra info: graph of bugs and developers according to the criticality of the bug
    \item information on how the debuggers follow the proposed states shown in Section 3
    \item time distribution at the different states
\end{itemize}

\subsection{Numerical results}
Results comparing the emiprical data with the analytic model are shown in Fig.~\ref{fig:closed-dist}.  
%The plotted transient probability of node/state $\tt 5D$, $P_{5D}(t)$ is the cumulative distribution function (CDF), $F(t)$ of the software bug resolve time. 
%
% \begin{figure}[htb]
%     \centering
%     \includegraphics[angle=-90,width=\columnwidth]{figs/response-time.pdf}
%     %\caption{Transient probabilities for three of the states in the ONAP case, $p_{10}(t)$ is the cumulative resolve time distribution (CDF)}\label{fig:resp-time}
%     \caption{Cumulative resolve time distribution (CDF)}\label{fig:resp-time}
% \end{figure}

% \begin{figure*}[tb]%
% \centering
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-ONOS, pri=1.pdf}
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-ONAP, pri=1.pdf}
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-Apache,pri=1.pdf}\\
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-ONOS, pri=2.pdf}
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-ONAP, pri=2.pdf}
% \includegraphics[width=0.66\columnwidth]{plots/closed-dist-Apache,pri=2.pdf}
% \caption{Comparison of the empirical cumulative resolve time distribution (CDF) the analytic model model for three projects and two priority levels. \poul{Too many, they all show the same, we need to select two (or four?)}}%
% \label{fig:closed-dist}%
% \end{figure*}




==> commands_acm.tex <==
% From The ACM Publishing System (TAPS) List of Accepted LaTeX Packages
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage[]{units}
\usepackage{multirow}

% conflict between amssymb and newtxmath https://tex.stackexchange.com/questions/564075/can-newtxmath-be-used-with-amssymb-in-pdflatex
% \let\Bbbk\relax
% \usepackage{amssymb}

% Not in The ACM Publishing System (TAPS) List of Accepted LaTeX Packages
\usepackage{import}
\usepackage{nameref}
%\usepackage{url}
\usepackage{flushend}
%\usepackage{changes} %gives error
\usepackage{enumerate}% http://ctan.org/pkg/enumerate
\usepackage[np]{numprint}
\usepackage{comment}
% *** SPACE TRICKS ***
\usepackage{setspace}

% \setaddedmarkup{\textcolor{red}{#1}}
% \npstyleenglish
%\usepackage{caption}

% For comments in the text:
\newcommand{\poul}[1]{\textcolor{blue}{PH: #1}}
\newcommand{\cmas}[1]{\textcolor{red}{ #1}}
\newcommand{\yagiz}[1]{\textcolor{green}{ZO: #1}}


% Definition environment
\newtheorem{definition}{Definition}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\renewcommand{\dbltextfloatsep}{3pt}
\renewcommand{\textfloatsep}{3pt}

